Mining Subjectively Interesting Attributed Subgraphs

Community detection in graphs, data clustering, and local pattern mining are three mature fields of data mining and machine learning. In recent years, attributed subgraph mining is emerging as a new powerful data mining task in the intersection of these areas. Given a graph and a set of attributes for each vertex, attributed subgraph mining aims to find cohesive subgraphs for which (a subset of) the attribute values has exceptional values in some sense. While research on this task can borrow from the three abovementioned fields, the principled integration of graph and attribute data poses two challenges: the definition of a pattern language that is intuitive and lends itself to efficient search strategies, and the formalization of the interestingness of such patterns. We propose an integrated solution to both of these challenges. The proposed pattern language improves upon prior work in being both highly flexible and intuitive. We show how an effective and principled algorithm can enumerate patterns of this language. The proposed approach for quantifying interestingness of patterns of this language is rooted in information theory, and is able to account for prior knowledge on the data. Prior work typically quantifies interestingness based on the cohesion of the subgraph and for the exceptionality of its attributes separately, combining these in a parametrized trade-off. Instead, in our proposal this trade-off is implicitly handled in a principled, parameter-free manner. Extensive empirical results confirm the proposed pattern syntax is intuitive, and the interestingness measure aligns well with actual subjective interestingness.

==> tex/interestingness.tex <==
\section{Interestingness of patterns\label{sec:interestingness}}
In order to assess the interestingness of an \pattern{s} $F$, we use the framework of interesting pattern mining introduced by De Bie \cite{DBLP:conf/kdd/Bie11,DBLP:journals/datamine/Bie11}. This framework is based on modelling the user's prior belief state about the data by means of a Maximum Entropy (MaxEnt) distribution, subject to any stated prior beliefs the user may hold about the data. This distribution is referred to as the background distribution. The interestingness of a pattern is then formalised by contrasting the pattern with this background distribution, as the ratio of two quantities:
\begin{itemize}
\item the self-information of the pattern, defined as minus the logarithm of the probability that the pattern is present under the background distribution, and
\item the description length of the pattern, which should formalise the amount of effort the user needs to expend to assimilate the pattern.
\end{itemize}
The interestingness of $F$ can be then expressed by the equation of information ratio $IR$:
$$
IR(F)=\frac{SI(F)}{DL(F)}
$$
Where $SI(F)$ represents the self-information of $F$, while $DL(F)$ is the description length of $F$. We first present how $SI(F)$ is calculated, then we define the function $DL(F)$.
\subsection{Self-information} \label{selfInfo}


The self-information of a pattern is calculated in a similar way to \cite{DBLP:journals/ijdsa/LijffijtSKB16}, but we only consider the relationship $\mathcal{R}_1$ between vertices entity type $E_1$ and attributes entity type $E_2$. We can represent $\mathcal{R}_1$ by a matrix $D_R$ with $|E_1|$ rows and $|E_2|$ columns. The relationship $\mathcal{R}_1$ is incoded in $D_R$ by ensuring that $D_R(i_1,i_2)=1$ iff $(e_{i_1},e_{i_2}) \in \mathcal{R}_1$. Then the prior information on the relationship type $R$ can be expressed as sums of $D_R$ columns, and sums of $D_R$ rows:

\begin{equation*}
\left\lbrace
\begin{array}{l}
 \sum_{D_R} P_R(D_R) \sum_{j=1}^{|E_2|} D_R(i,j)= \sum_{j=1}^{|E_2|} D_R(i,j)  \forall i \in \llbracket 1, |E_1| \rrbracket  \\
  \sum_{D_R} P_R(D_R) \sum_{i=1}^{|E_1|} D_R(i,j)= \sum_{i=1}^{|E_1|} D_R(i,j)  \forall j \in \llbracket 1, |E_2| \rrbracket 
\end{array}
\right.
\end{equation*}
Since $P_R$ is a probability distribution, it needs to be normalized, which gives the constraint: $\sum_{D_R} P_R(D_R)=1$. The MaxEnt optimization problem maximizes $\sum_{D_R} -P_R(D_R)log(P_R(D_R))$, the entropy, with respect to $P_R$, subject to the above constraints. As shown in \cite{DBLP:journals/datamine/Bie11}, the optimal solution is of the form:
$$
P_R(D_R)=\prod_{i_1,i_2} P_R^{ \{ i_1,i_2  \} }  D_R(i_1,i_2)
$$
where: $P_R^{\{ i_1,i_2  \}} (d)=\frac{exp(d \times \sum_{t} \lambda_R^{t,i_t} )}{1+exp( \sum_{t} \lambda_R^{t,i_t} )}$. $\lambda_R^{t,i_t}$ is a Lagrange multiplier corresponding to the constraint for entity $i_t$ of type $t$. The optimal values of these multipliers can be found by solving the convex Lagrange dual optimization problem. Then, we can define the function $SI(F)$ as:
$$
SI(F)=- \sum_{e_i \in F \cap E_1} \sum_{e_j \in F \cap E_2} log(P_R^{ \{ i,j \} } (1)) 
$$
where $P_R^{\{i,j\}} (1)$ signifies the probability that the relation $(e_i,e_j)$ exists. 


\subsection{Description length} \label{descLength}
Considering that the goal is to describe the pattern $F$ based on intersection of neighborhoods (represented by the elements in $E_3$), we need to define a function that quantifizes the length of such a description. Although we already have a potential description $F \cap E_3$, it may not be the best, other possible descriptions could be the subsets $F_3 \subseteq F \cap E_3$ . One aims to find a description that contains the minimum of entities from $F \cap E_3$, and that covers the maximum of vertices corresponding to  entities $F \cap E_2$. This can be quantified by the function $f:E_3 \times E_1 \longrightarrow \mathbb{R}$ defined for $F_3 \subseteq E_3$ and $F_1 \subseteq E_1$ as:
$$
f(F_3,F_1)=(|F_3|+1) \times log(|E_3|)+(|errors(F_3,F_1)|+1) \times log(|E_1|)
$$
With: 
$$error(F_3,F_1)= \cap_{e \in F_3} map(e) - \cup_{e \in F_1} map(e)  $$
In other terms, $f$ computes the number of bits required to specify the entities of $F_3$, plus the number of bits required to specify the errors: the vertices that belong to the intersection of neighborhoods in $F_3$ but not to the vertices associated to $F_1$ entities. Finally, $DL(F)$ is calculated based on the description that minimizes $f$:

$$
DL(F)=\min_{F' \subseteq F \cap E_3} f(F',F \cap E_1)
$$ 

This means that each found \pattern{} $F$ will be provided to the end-user with its minimum description defined by the following function: $MinD(F)=argmin_{F' \subseteq F\cap E_3} f(F',F \cap E_1)$.

\modif{ Would it be interesting to prove that calculating MinD(F) is an NP Complet problem? }







